Poster: Self-Supervised Quantization-Aware Knowledge Distillation

Quantization-aware training (QAT) starts with a pre-trained full-precision model and performs quantization during retraining. However, existing QAT works require supervision from the labels and they suffer from accuracy loss due to reduced precision. To address these limitations, this paper proposes a novel Self-Supervised Quantization-Aware Knowledge Distillation framework (SQAKD). SQAKD first unifies the forward and backward dynamics of various quantization functions and then reframes QAT as a co-optimization problem that simultaneously minimizes the KL-Loss and the discretization error, in a self-supervised manner. The evaluation shows that SQAKD significantly improves the performance of various state-of-the-art QAT works. SQAKD establishes stronger baselines and does not require extensive labeled training data, potentially making state-of-the-art QAT research more accessible.

==> ablation.tex <==
\section{Ablation Study}
\label{sec:ablation}





\subsection{Loss}

% \subsection{Effect of $\alpha$}

\subsection{Effect of Temperature $T$}

% Apprentice: Using KD Techniques to Improve Low-Precision Network Accuracy
% Although we did not do extensive studies experimenting with training on soft targets as opposed to logits, we did find that τ = 1 gives us best results when training on soft targets. Hinton et al. (2015) mention that when the student network is significantly smaller than the teacher network, small values of τ are more effective than large values.


\subsection{Effect of Initialization}

\subsection{Effect of training time}
EWGS 

\subsection{Different forward and backward combinations}
\kaiqi{Decouple the forward and backward propagation, investigate the performance}
To show the flexibility of our framework.
We find out that the success of EWGS is mainly due to its integration of the discretization error, defined as $x_c-x_q$, within the gradient approximation process (to be discussed in Section~\ref{sec:ablation}).

\subsection{Different Teacher Networks}
AIT
Different teacher model
Ensemble of teachers

\subsection{Different Teacher Pre-training Algorithms}
AIT

% \subsection{}
% \subsection{}
% \subsection{}

==> background.tex <==
% \section{Background and Related Works}
\section{Background and Related Works}




\subsection{Quantization}
Quantization is a promising approach for reducing the computational overhead of large full-precision models without altering the model structure~\cite{kim2022understanding}.
% Post-Training Quantization (PTQ)~\cite{liu2021post} applies quantization to model weights after training, 
Post-Training Quantization (PTQ)~\cite{liu2021post} directly quantizes a pre-trained model without extensive training, so it often results in accuracy degradation, especially in low-bit-precision quantization.
In contrast, Quantization-Aware Training (QAT)~\cite{sakr2022optimal} also starts with a pre-trained model but performs quantization during retraining which can mitigate the impact of quantization on model accuracy.
%Compared to PTQ, QAT mitigates the impact on model accuracy, but it is more computation-intensive due to the extra training~\cite{huang2023efficient}.
%The work in this paper falls under the QAT category, aiming to enhance the performance of quantized models through integrated quantization during training.

% Efficient Quantization-aware Training with Adaptive Coreset Selection:
% In addition, the quantization methods can also be classified as quantization-aware training (QAT) [9, 11, 12] and post-training quantization (PTQ) [33, 34, 35] based on whether to retrain a model with quantized weights and activations or start with a pre-trained model and directly quantize it without extensive training. QAT can better retrain the performance and works with extremely low-precision quantization such as 2-bit, while PTQ can only achieve 8-bit and 6-bit quantization. However, QAT is more computation-intensive due to the extra training. In this work, we focus more on the efficiency of QAT methods.



Early works on QAT, such as BNN~\cite{courbariaux2016binarized} and XNOR-Net~\cite{rastegari2016xnor} demonstrate the effectiveness of binary models on simple models and datasets.
%, where activations and weights are both quantized to 2 bits by introducing channel-wise scaling in the forward propagation.
These approaches quantize both activations and weights to 2 bits and introduce channel-wise scaling in the forward propagation.
% However, these approaches cause significant accuracy degradation when applied to large datasets~\cite{zhou2016dorefa, choi2018pact}, e.g., ImageNet.
However, when applied to large datasets like ImageNet, these methods suffer from significant accuracy degradation~\cite{zhou2016dorefa, choi2018pact}.
%
DoReFa-Net~\cite{zhou2016dorefa} improves upon these early works and shows that low-bit models can achieve comparable prediction accuracy to their 32-bit counterparts on ImageNet. 
Instead of channel-wise scaling, DoReFa-Net employs a constant scalar to scale all filters in the forward pass.
%
% Rather than using a constant scaling factor, PACT~\cite{choi2018pact} makes the clipping scalar a learnable parameter that is optimized during training to find the right quantization scale. 
%
% Continue in this direction, recent works make the quantization function learnable by introducing various parameters for controlling, 
\kai{The quantization function converts continuous-valued weights or activations to a discrete set of values.}
% It first clips the input into a smaller range, producing quantization intervals, and then converts the continuous quantization intervals into discrete values with the target quantization levels.
Recent works make the quantization function\m{explain what is this function} learnable by introducing trainable parameters that can be optimized during training.
These trainable parameters enable improved control over critical aspects of the quantization function, such as clipping ranges (PACT~\cite{choi2018pact}, LSQ~\cite{esser2019learned}, APoT~\cite{li2019additive}, and DSQ~\cite{gong2019differentiable}) \kai{i.e., the bounds within which the input values are constrained}, quantization intervals (QIL~\cite{jung2019learning} and EWGS~\cite{lee2021network})), \kai{i.e., the step size between adjacent quantization levels}, and quantization levels (LQ-Nets~\cite{zhang2018lq})\m{explain what these terms are}, \kai{i.e., the discrete representation of the original continuous values}.


% The quantization function maps continuous-valued weights or activations to a discrete set of values. It involves partitioning the range of values into quantization levels, with clipping ranges limiting the values within a specified range. Quantization intervals determine the spacing between levels.


% However, these varying algorithms cannot be generalized and it is unclear how to improve them. 
% However, the aforementioned quantization algorithms are motivated by varying heuristics and it is unclear how to improve them.
% This paper proposes a generalized framework, attempting to close this gap.
However, the aforementioned quantization algorithms are driven by varying heuristics, and \kai{there is a lack of a generalized framework}\m{this is too vague \kai{Changed ``clarity on how'' to ``a generalized framework''}} to further improve them. 
This paper aims to close this gap by providing a generalized framework that can enhance the existing quantization approaches.
%
% In addition, it is worth mentioning that the work in MQbench~\cite{} shows that the difference between quantization algorithms is not as significant as reported in the original paper, and no algorithm achieves the best or the worst performance on every architecture.
% Therefore, an easy-to-implement, effective, generalized framework that can improve the existing quantization approaches is more necessary than a method that can work perfectly on all the model architectures and all the datasets.
In addition, it is worth to note the findings from MQbench~\cite{li2021mqbench} which indicate that the difference between quantization algorithms is not as substantial as reported in the original \kai{papers}\m{papers?};
and no algorithm achieves the best or the worst performance on every architecture~\cite{li2021mqbench}. 
Therefore, motivated by this, we argue that, there is a need for an easy-to-reproduce, effective, and generalized framework that can improve the performance of existing quantization methods.
%
% Furthermore, while the existing approaches perform well for high-bit quantization (4 bits or more), however, the low-bit network (1-3 bits) suffers a severe accuracy drop, as shown in Figure~\ref{}.
% This paper tries to improve the quantized network with low-bit precision.
% Furthermore, while existing approaches perform well for high-bit quantization (4 bits or more), they often suffer from a substantial accuracy drop when applied to low-bit networks (1-3 bits), as illustrated in Figure~\ref{}. 
Furthermore, the aforementioned top-performing quantization algorithms all involve high-bit networks (4 bits or more), with, however, little attention on low-bit networks (1-3 bits). 
Empirically, we find that existing techniques do not work well on low-bit networks. 
Our proposed framework aims to improve the performance of both low-bit and high-bit precision quantized networks.
\kaiqi{Check whether the performance drops when low bit, and use a table or figure to show it.}
\m{should you also mention the self-supervised aspect of your work? \kai{How about mentioning it in the subsection C?}}

% The aforementioned top-performing SSL algorithms all involve large networks (e.g., ResNet-50 (He et al., 2016) or larger), with, however, little attention on small networks. 
% Empirically, we find that existing techniques like contrastive learning do not work well on small networks. 
% For instance, the linear probe top-1 accuracy on ImageNet using MoCo-V2 (Chen et al., 2020c) is only 36.3\% with MobileNet-V3-Large (see Figure 1), which is much lower compared with its supervised training accuracy 75.2\% (Howard et al., 2019).

% However, these algorithms cannot be generalized for the arbitrary codebooks and it is unclear how to extend them. Our paper closes this gap.

% ======= Summary Notes
% PACT~\cite{choi2018pact}, LSQ~\cite{esser2019learned}, DoReFa~\cite{zhou2016dorefa}, and EWGS~\cite{lee2021network}
% EWGS: learn lower and upper bounds of quantization intervals
% APoT: an efficient non-uniform quantization scheme for the bell-shaped and long-tailed distribution of weights and activations in neural networks.






% \subsubsection{Knowledge Distillation (KD)}
\subsection{Knowledge Distillation (KD)}
KD aims to improve the performance of small, fast networks (termed ''student'') by transferring knowledge from large, cumbersome networks (termed ''teacher'') during training.
%
Various KD techniques~\cite{hinton2015distilling,romero2014fitnets,zagoruyko2016paying,tung2019similarity,peng2019correlation,ahn2019variational,park2019relational,passalis2018probabilistic,heo2019knowledge,kim2018paraphrasing,yim2017gift,huang2017like} have been investigated for different image classification models.
%
Hinton et al. first introduce transferring soft logits (softmax outputs)~\cite{hinton2015distilling} by minimizing the Kullback–Leibler (KL) divergence between the teacher's and student's soft logits and the cross-entropy loss with the data labels. 
%
Later, other works~\cite{romero2014fitnets,zagoruyko2016paying,tung2019similarity,peng2019correlation,ahn2019variational,park2019relational,passalis2018probabilistic,heo2019knowledge,kim2018paraphrasing,yim2017gift,huang2017like} propose to transfer various forms of intermediate representations, such as FSP matrix~\cite{yim2017gift} and attention maps~\cite{zagoruyko2016paying}.
These works assume that the output dimensions of intermediate layers are independent, and they let the student replicate the teacher's behavior by minimizing the difference between their probabilistic outputs. 
However, the intermediate representations are interdependent, and this minimization fails to capture the important structural knowledge of the teacher's convolution layers.
%
To address this problem, recent works, e.g., CRD~\cite{tian2019contrastive} and CKTF~\cite{zhao2023contrastive}, formulate KD as optimizing contrastive objectives, usually used for representation learning~\cite{van2018representation, gutmann2010noise, chen2020simple, tian2020makes}.
However, despite the success of KD techniques in developing efficient image classification models, there has been limited understanding of KD on the model quantization~\cite{kim2022understanding}.


% \subsubsection{Knowledge Distillation + Quantization}
% Despite the success of KD techniques in developing efficient image classification models, there is a lack of comprehensive analysis and understanding of KD in the context of QAT.
% We are the first to 1) quantitatively investigate the performance of diverse KD techniques in assisting QAT to minimize the accuracy disparity between the quantized student and the full-precision teacher,
% and 2) provide an in-depth analysis of the loss surface of KD within QAT.
% \kaiqi{Will add virtualization of the loss surface in Evaluation}

% Understanding and Improving Knowledge Distillation for Quantization-Aware Training of Large Transformer Encoders:
% Although these KD-based compression techniques have developed efficient BERT structures, there has been limited understanding of KD on the model quantization. In particular, we are the first to quantitatively reveal that more distillation of the intermediate representations helps QAT reduce the accuracy gap between the quantized student and the full-precision teacher.



% \subsection{Knowledge Distillation + Quantization}


\subsection{Knowledge Distillation + Quantization}
\label{sec:related_works_KD_and_QAT}


% QKD~\cite{kim2019qkd}, CMT-KD~\cite{pham2023collaborative}, SPEQ~\cite{boo2021stochastic}, and PQ+TS+Guided~\cite{zhuang2018towards}.



\begin{table*}[t]
% \setlength{\tabcolsep}{6.pt}
\centering
\caption{Summary of related works that employ KD to enhance the training of low-precision networks.
The training cost is estimated by considering the time required for training the pre-trained teacher ($N \times T_{pre}$) during initialization and the training time for the teacher ($M_t \times T_t$) and student ($M_s \times T_s$) during quantization-aware training with KD, 
where $N$ denotes the number of pre-trained teachers, $M_t$ and $M_s$ denote the number of training phases for the teacher and student, respectively.
If the approach involves joint training of the teacher and student, $M_t \times T_t$ is added to the total training time; otherwise, it is not included.}
\label{tab:summary_related_works}
\begin{tabular}{@{}lllllll@{}}
\toprule
               & \begin{tabular}[c]{@{}l@{}}Self-\\ Supervised\end{tabular} & \begin{tabular}[c]{@{}l@{}}Number\\ of hyper-\\ parameters\\ for balancing \\ loss terms\end{tabular} & \begin{tabular}[c]{@{}l@{}}Number of \\ training \\ phases\end{tabular} & Training cost            & Initial teacher type                  & \begin{tabular}[c]{@{}l@{}}Train jointly / \\ Train the student only\end{tabular} \\ \midrule
AP-SCHEME-A~\cite{mishra2017apprentice}    & No                                                         & 3                                                                                                     & 1                                                                       & $T_{s} + T_{t}$          & One random initialized full-precision & Train jointly                                                                     \\
AP-SCHEME-B~\cite{mishra2017apprentice}    & No                                                         & 3                                                                                                     & 1                                                                       & $T_{pre}+T_{s}$          & One pre-trained full-precision        & Train the student only                                                            \\
AP-SCHEME-C~\cite{mishra2017apprentice}    & No                                                         & 3                                                                                                     & 2                                                                       & $T_{pre} + 2T_{s}$      & One pre-trained full-precision        & Train the student only                                                            \\
QKD~\cite{kim2019qkd}            & No                                                         & 2                                                                                                     & 3                                                                       & $T_{pre}+3T_{s}+T_{t}$  & One pre-trained full-precision        & Train jointly                                                                     \\
CMT-KD~\cite{pham2023collaborative}         & No                                                         & 3                                                                                                     & 1                                                                       & $NT_{pre}+T_{s}+T_{t}$  & Multiple different bit-widths         & Train jointly                                                                     \\
SPEQ~\cite{boo2021stochastic}           & No                                                         & 1                                                                                                     & 1                                                                       & $T_{pre}+T_{s}+T_{t}$    & One quantized with target bit-width   & Train jointly                                                                     \\
PQ+TS+Guided~\cite{zhuang2018towards}   & No                                                         & 2                                                                                                     & 4                                                                       & $T_{pre}+4T_{s}+T_{t}$  & One pre-trained full-precision        & Train jointly                                                                     \\
\textbf{SQAKD (Ours)} & \textbf{Yes}                                               & \textbf{0}                                                                                            & \textbf{1}                                                              & $\mathbf{T_{pre}+T_{s}}$ & One pre-trained full-precision        & Train the student only                                                            \\ \bottomrule
\end{tabular}
\end{table*}





% \kaiqi{labels are necessary, complicated training process, hyper-parameter tuning}


Several recent works~\cite{mishra2017apprentice, kim2019qkd, boo2021stochastic, zhuang2018towards, pham2023collaborative} have employed KD to enhance the training of low-precision networks, where the low-precision network acts as the student and the high-precision or full-precision network serves as the teacher.
% In Apprentice (AP)~\cite{mishra2017apprentice}, Mishra et al. propose three schemes of applying KD to improve the ternary-precision or 4-bit network.
Mishra et al. proposed three schemes in Apprentice (AP) for improving ternary-precision or 4-bit networks.
QKD~\cite{kim2019qkd} coordinates quantization and KD through three phases, including self-studying, co-studying, and tutoring.
SPEQ~\cite{boo2021stochastic} constructs the teacher by sharing the model parameters of the student and assigns stochastic bit precision to the teacher's activations.
PQ+TS+Guided~\cite{zhuang2018towards} proposes a 4-stage training strategy, including a two-stage optimization strategy of first optimizing quantized weights and then quantized activations, a progressive optimization approach to progressively decreases the bit width, and a learning scheme of jointly training a full-precision teacher alongside the low-precision student.
CMT-KD~\cite{pham2023collaborative} encourages both collaborative learning between quantized teachers and mutual learning between quantized teachers and the quantized student.



We summarize the features of the aforementioned works in Table~\ref{tab:summary_related_works}. 
Despite their contributions, they possess multiple drawbacks.
% , as their features are summarized in Table~\ref{tab:summary_related_works}. 
%
First, they all require a delicate balance for the weights of different loss terms, which leads to tedious hyper-parameter tuning. 
For example, in QKD, three hyper-parameters are required for balancing loss terms, and their influence on performance is substantial.
%
Second, all the existing works are developed under a strong assumption that labels of the training data are always available during the training of QAT, 
% whereas insufficient labeled data can often happen in real-world applications.
whereas access to a sufficient amount of labeled data can be limited or costly in real-world scenarios.
%
% Third, they require a complex, cost-expensive training process, leading to difficulty in reproducing and deployment.
Third, they require a complex, computationally expensive training process, e.g., 3 training phases required in QKD and a 4-stage optimization strategy proposed in PQ+TS+Guided, posing challenges in reproducibility and deployment feasibility.
%
Finally, these works tend to focus on one specific KD approach alongside one particular quantization function, lacking a comprehensive evaluation and analysis of varying KD techniques within the context of QAT.
%
In contrast, this paper 1) quantitatively investigates the performance of diverse KD techniques in assisting QAT with different quantizers,
2) provides an in-depth analysis of the loss surface of KD within QAT,
% and 3) proposes a novel quantization-aware KD method, which does not require hyper-parameters for balancing loss terms, is self-supervised (no labels are required), simple-to-reproduce, low training cost, as discussed in the rest of the paper.
and 3) proposes a novel quantization-aware KD framework, which eliminates the need for hyper-parameter balancing, operates in a self-supervised manner without labeled data, is applicable to incorporate various quantizers, and offers simplicity in reproducibility and reduced training cost.
% as discussed in the rest of the paper.
\kaiqi{Will add virtualization of the loss surface in Evaluation}


% from several aspects, including whether it is self-supervised, the number of hyper-parameters for balancing loss terms, the number of training phases, and the training cost which is estimated by the initial teacher type, and training the teacher or student jointly or train the student only.

% This paper proposes an MR-based KD method tailored for ASR models and employing a novel nonlinear replacing rate scheduler, as discussed in the rest of the paper.


% Despite the success of KD techniques in developing efficient image classification models, there is a lack of comprehensive analysis and understanding of KD in the context of QAT.
% We are the first to 1) quantitatively investigate the performance of diverse KD techniques in assisting QAT to minimize the accuracy disparity between the quantized student and the full-precision teacher,
% and 2) provide an in-depth analysis of the loss surface of KD within QAT.
% \kaiqi{Will add virtualization of the loss surface in Evaluation}

==> conclusion.tex <==
\section{Conclusion}

This paper proposes

==> discussion.tex <==
%\section{Discussion}


